Particle identification performance of the prototype Aerogel RICH counter for the Belle II experiment

We have developed a new type of particle identification device, called an Aerogel Ring Imaging Cherenkov (ARICH) counter, for the Belle II experiment. It uses silica aerogel tiles as Cherenkov radiators. For detection of Cherenkov photons, Hybrid Avalanche Photo-Detectors (HAPDs) are used. The designed HAPD has a high sensitivity to single photons under a strong magnetic field. We have confirmed that the HAPD provides high efficiency for single-photon detection even after exposure to neutron and gamma-ray radiation that exceeds the levels expected in the 10-year Belle II operation. In order to confirm the basic performance of the ARICH counter system, we carried out a beam test at the DESY using a prototype of the ARICH counter with six HAPD modules. The results are in agreement with our expectations and confirm the suitability of the ARICH counter for the Belle II experiment. Based on the in-beam performance of the device, we expect that the identification efficiency at 3.5 GeV/c is 97.4% and 4.9% for pions and kaons, respectively. This paper summarizes the development of the HAPD for the ARICH and the evaluation of the performance of the prototype ARICH counter built with the final design components.

==> 6_conclusion_v3.0.tex <==
We have developed a proximity-focusing RICH counter with an aerogel radiator, i.e. an ARICH counter, as a new particle identification device in the Belle II experiment. 
We use a HAPD as the Cherenkov photon detector of the ARICH counter.
The tolerance to neutron and $\gamma$-ray irradiation is a very important issue for a photon detector.
By improving the HAPD design, the HAPDs have become sufficiently radiation tolerant for reliable 10-year Belle II operation.

In order to confirm the basic performance of the ARICH counter using the designed components, we carried out a beam test of a prototype.
We measured, on average, $10.495 \pm 0.111$ photoelectrons per track, with a single-photon resolution of \unit{14.03}{mrad}.
We estimate a 5.47 $\sigma$ separation between pions and kaons using this prototype ARICH counter.

To estimate the performance of the $\pi/K$ identification, we analyzed the simulated data by employing the likelihood method using a PDF from the beam test data.
The resulting $\pi$ and $K$ identification efficiency was estimated at 97.4\% and 4.9\%, respectively, with the cutoff for a likelihood ratio of 0.2 at \GeV{3.5}.

==> 7_acknowledgment_v4.0.tex <==
This study was partially supported by a Grant-in-Aid for Scientific Research (A) (No.24244035) from the Japan Society for the Promotion of Science (JSPS).
We would like to thank Hamamatsu Photonics K.K. for their support in equipping the HAPDs.
We would like to thank the J-PARC MLF staff, Nagoya University, especially the High Energy Physics Group, and the DESY staff for their support in the irradiation tests and the beam test.
We also thank the graduate students of Niigata University, Tokyo University of Science, Toho University, and Tokyo Metropolitan University for their assistance.
